Online FDR Control for RNAseq Data

Motivation: While the analysis of a single RNA sequencing (RNAseq) dataset has been well described in the literature, modern research workflows often have additional complexity in that related RNAseq experiments are performed sequentially over time. The simplest and most widely used analysis strategy ignores the temporal aspects and analyses each dataset separately. However, this can lead to substantial inflation of the overall false discovery rate (FDR). We propose applying recently developed methodology for online hypothesis testing to analyse sequential RNAseq experiments in a principled way, guaranteeing FDR control at all times while never changing past decisions. Results: We show that standard offline approaches have variable control of FDR of related RNAseq experiments over time and a naively composed approach may improperly change historic decisions. We demonstrate that the online FDR algorithms are a principled way to guarantee control of FDR. Furthermore, in certain simulation scenarios, we observe empirically that online approaches have comparable power to offline approaches. Availability and Implementation: The onlineFDR package is freely available at http: //www.bioconductor.org/packages/onlineFDR. Additional code used for the simulation studies can be found at https://github.com/latlio/onlinefdr_rnaseq_simulation

==> comments.tex <==
AO 1
I find this argument not to be very convincing and distracting form the key value of your method. Realistically RNAseq in target discovery drives a very small portion of decision making, and typically only top and most convincing results are progressed to next steps. Also, all expression studies need to be functionally validated experimentally and on protein level to make it as far as an FIH. 
[Lathan] I think this comment has merit, and we can perhaps motivate this in a different way. 

Importantly, I think the key value of the approach is actually to allow to dig deeper in the data and expand the space of potential targets for validation; and extend the potential for novel discovery, i.e. find targets we would have missed otherwise. And targets we would be missing cannot be already failing in clinical trials, since we’re not pursuing them.
[Lathan] I think this fundamentally missed the mark. However, she's not alone -- other scientists we've spoken to have also raised similar points. I don't think this is necessarily a challenge our paper has to solve (it's a big challenge). The key is to really motivate the need for false discovery rate control (e.g. DECREASING, not expanding, the space of potential targets for validation). And then, IF WE GET COMPARABLE POWER, that's a by-product as opposed to a primary outcome. Otherwise this comment is like trying to fit a square peg into a circular hole; it's talking about something entirely different (Type I errors vs. Type II errors).
[Milena] I agree with the first part of AO1, the second part has indeed missed some of the concepts. However, I would recommend to delete this whole part. It is not needed and provides no “need to know” information.
 
AO 2
It would be good to be more precise around that a “related” RNAseq experiment is. Does it need to have the same design? Shared controls / biological replicates? Or can it be something quite distant (and with high heterogeneity) e.g. grouping all chemotherapy - treated samples across tumor types, regardless of specific chemotherapeutic agent, patient demographics, etc. 
[Lathan] Done.
 
AO 3
I think TCGA or any other consortium would be a good case study of RNAseq data where you keep adding samples over time. So let’s say in a consortium you start with sample type A and only 2 samples per treatment group, and you make a set of conclusions. In half a year you have 15 samples in each group and conclusions will change as the power of your study is now greater. Why wouldn’t we want to change the conclusions we made on the 2 samples when the comparison was severely underpowered?
In other words - are there upper and lower limits for sample counts for when you’d advise to start using online FDR?

I think this is an important point to clarify the addition of samples vs. the addition of datasets. I agree that if samples are added, then your point holds true. It's the latter case that for which online methods are motivated. GEO is perhaps a more representative real-world example of datasets that are uploaded into a central repository.
 
AO 4
Please clarify the hypothesis batching - maybe it’s later in the text, but in the introduction it’s not explained at all.
[Lathan] Great comment, added some explanatory text.
 
AO 5 in text
[Lathan] Done.
 
AO 6 
Up until this point it’s not mentioned online will also use BH. Is it for comparison only. Then in the procedure - “order p-values” is that across all samples from historic + current data? Maybe mention the combination of RNAseq datasets first?
[Lathan] In the section where you make this comment, we haven't discussed online yet. Section 2.2 is nothing new. This is what everyone knows. You order p-values in the data you have. It doesn't make sense to talk about online first. You need to at least understand what is currently done (which we are calling offline) in order to understand online. Think of the online method as a principled way of applying Benjamini-Hochberg again and again. Let's say we have three datasets. We compare offline Benjamini-Hochberg where we apply Benjamini Hochberg 3 times, pooled offline BH assuming that we made one giant dataset and applied Benjamini Hochberg once, and then online where we apply benjamini hochberg technically 3 times, but in this mathematically principled way. 
 
AO 7
As in are generated from independent experiments? Independent samples? Is that assumption defining any requirements for when the method should be used? I.e. should we use BatchPRDS for dependent p-values.
[Lathan] Correct to use BatchPRDS for dependent p-values.
 
AO 8 
Do the batch 1, 2, 3 use the same animals/animal models, or all have different animals?
[Lathan] I believe these are same type of mouse, but different mouse samples. We already discuss this later in the manuscript.
 
AO 9
Would be nice to see total number of hypotheses (genes) tested for each, or a %. 
[Lathan] Good suggestion. Done.

Also maybe separate table into two subsections of online / offline methods. 
Also, very minor difference between offline and pooled offline - why is the comparison relevant to show?
[Lathan] Just because difference is small doesn't mean that it's no longer relevant...we motivate this earlier in the paper.

The table shows two main trends - increase in rejections with batches (can it be explained by sample size alone? Maybe you’ll show in simulations later, but it would be interesting to factor in and discuss the sample size and resulting rejections); and decrease in rejections from uncorrected to offline to batch. What is difficult to tell if there is any interaction between these two. 
[Lathan] It's unsurprising that the number of rejections will increase with number of batches (i.e. number of hypotheses being tested -> number of pvalues). I think a more interesting discussion point is whether the number of experimental samples - THIS IS DIFFERENT FROM NUMBER OF PVALUES (we've used 5 control and 5 experimental) in our simulations is associated with online control FDR and power. Without ground truth, we cannot make any conclusions about power or FDP. The main takeaway I have at least is that Batch procedures are rejecting fewer hypotheses. This should make readers think that we're controlling the false discovery rate at least more stringently than offline approaches and obviously more than uncorrected. 
 
AO 10
It’s nice to see detailed data, however in similar vein to the previous comment, it would be good to see a simplified summary, e.g. with barplot of key trends (overlap increase/discrease by method or batch)
Thanks for the comment. 
 
AO 11
I am not convinced about the changing of historic decisions comment as it lacks an argument for why it’s bad (besides intuition). What if my new sample batches are bigger or collected with improved technology. 
[Lathan] I'm finding this tough to substantiate. It seems so obvious to me that changing history is bad...Just because your future is improved doesn't mean that you need to change the decisions you already made, or should even.
 
AO 12 
I don’t agree with this statement. Differences from even low expression values to zero show very high DE.
[Lathan] Thanks! Removed this statement.
 
AO 13 
I would avoid making an argument about 2-group comp being most common. In my experience it’s not.
[Lathan] Thanks! Removed this statement.

AO 14
Fig 3. I’m really struggling to differentiate the colors, to the point of not being able to interpret the graph. Mostly challenging with the shades of brown. Also the legend colors could be bigger.
Similarly to earlier comment, some form of visual grouping of methods by offline and online could help follow the story.
[Lathan] Thanks for your great suggestions!
 
AO 15
Please clarify the meaning of reordered batches and rationale to test it.
 
AO 16
Fig 4. Same as above about colors. Also, what is the confidence interval in plot A? Could be added to the legend.
[Lathan] Done.
 
 
General
I think some text in the paper I highlighted by accident, generally I write out the comments, so you can ignore the text highlights.

As a reader I would like more guidance on when it’s advisable to use the method in various real world settings, e.g. RNAseq consortia such a TCGA vs smaller focused studies, or clinical studies, especially since industry/academia are frequently mentioned. 

It may make sense for the simulation section to be before the real world dataset section. Or:
To be honest, I think the real world dataset section is the paper’s weak point because it invites a debate and questions on how the method impacts conclusions and their novelty. One approach would be to remove some of the claims on the ability of the method to improve decision making and also remove the real world example, focus on the method and simulations. Another would be to actually expand on the real world data to support the claim of novel biological findings somehow. Just that we have more/less genes in itself is meaningless to a computational biologist. In theory you could have fewer DE genes but they’re more coherent as members of key biological processes, and therefore lead to novel biological discoveries. A third in between approach would be to maybe test ability of the DEgene sets to discover enriched pathways, e.g. focusing on just a well curated set of pathways, e.g. HALLMARK from msigdb. That could potentially serve as a proxy to a novel biological discovery. 

